Massively Parallel Computation via Remote Memory Access

We introduce the Adaptive Massively Parallel Computation (AMPC) model, which is an extension of the Massively Parallel Computation (MPC) model. At a high level, the AMPC model strengthens the MPC model by storing all messages sent within a round in a distributed data store. In the following round, all machines are provided with random read access to the data store, subject to the same constraints on the total amount of communication as in the MPC model. Our model is inspired by the previous empirical studies of distributed graph algorithms using MapReduce and a distributed hash table service. This extension allows us to give new graph algorithms with much lower round complexities compared to the best known solutions in the MPC model. In particular, in the AMPC model we show how to solve maximal independent set in $O(1)$ rounds and connectivity/minimum spanning tree in $O(\log\log_{m/n} n)$ rounds both using $O(n^\delta)$ space per machine for constant $\delta < 1$. In the same memory regime for MPC, the best known algorithms for these problems require polylog $n$ rounds. Our results imply that the 2-Cycle conjecture, which is widely believed to hold in the MPC model, does not hold in the AMPC model.

==> algorithms.tex <==
\section{Algorithms}\label{sec:algorithms}

\input{two-cycle}
\input{mis}
\input{connectivity}
\input{spanning-forest}
\input{forest-connectivity}
\input{mst}


==> experiments.tex <==
\section{Empirical Study}\label{sec:experiments}
\newcommand{\ccalg}[0]{\textsc{ContractCC}}
In this section we provide a preliminary empirical study of the \AMPC{} model.
The goal of the study is to analyze whether the assumption that each machine can make up to $O(n^\epsilon)$ queries in a single round is realistic.

We study the \textsc{2-Cycle} problem, in which the input is a graph consisting of either a single cycle of length $n$ or two cycles of length $n/2$, and the algorithm has to find the number of cycles.
We compare an implementation of Algorithm~\ref{alg:twocycle} with the state-of-the-art implementation of the algorithm for finding connected components~\cite{cc-contractions}, which we call \ccalg{}.
Note that Algorithm~\ref{alg:twocycle} shrinks the number of vertices by roughly $n^\epsilon$ in each round, while \ccalg{} shrinks the number of vertices by a constant factor in each round.
As a result, Algorithm~\ref{alg:twocycle} runs in $O(1/\epsilon)$ rounds (Theorem~\ref{thm:twocycle}), while \ccalg{} requires $\Theta(\log n)$ rounds, which is inevitable under \textsc{2-Cycle} conjecture.

We implemented both algorithms in a proprietary framework implementing the \MPC{} model, which allows one to run sequences of MapReduce-like computations (similarly to Apache Spark~\cite{spark} and FlumeJava~\cite{flumejava}).
In order to implement the \AMPC{} capabilities, we run an external service providing distributed data storage capabilities (see e.g.~\cite{bigtablepaper}).
As a result, machines exchange data both by sending messages to each other (using the framework capabilities) and by using the DDS.
The DDS service does not take advantage of hardware support for RDMA.
We believe that using a framework that integrates \MPC{} with DDS capabilities and takes advantage of an optimized RDMA mechanism would yield noticeably smaller running times of our \AMPC{} algorithm.

We ran the experiments on a shared cluster, repeating each run X times.
The results are given in Table~\ref{tab:experiments}.


==> implementations.tex <==
\section{Implementation Details}\label{apx:implementation-details}

In this section we provide some details on the implementation of our
algorithm in $\AMPC{}$. We start by reviewing some known computational
primitives in the $\MPC{}$ model with strictly sublinear space per
machine.

\subsection{Primitives}
The following primitives can be implemented in the $\MPC{}$ model
using $O(n^{\epsilon})$ space per machine.  All of the algorithms here
use space proportional to the input to the primitive (denoted by $N$).
Note that the primitives below all run in $O(1/\epsilon)$ rounds in
the \MPC{} model, which implies $O(1/\epsilon)$ rounds in the \AMPC{}
model.

\begin{itemize}
\item {\bf Sorting.} Sorting $N$ tuples be solved in $O(1/\epsilon)$
rounds~\cite{DBLP:conf/isaac/GoodrichSZ11}. The input is a sequence of
$N$ tuples, and a comparison function $f$. The output is a sequence of
$N$ tuples that are in sorted order with respect to $f$.

\item {\bf Filtering.} Filtering $N$ tuples can be solved in
$O(1/\epsilon)$ rounds. The input is a sequence of $N$ tuples, and a
predicate function $f$. The output is a sequence of $k$ tuples such
that a tuple $x$ is in the output if and only if $f(x) =
\texttt{true}$.

\item {\bf Prefix Sums.} Computing the prefix sum of a sequence of $N$
tuples can be solved in $O(1/\epsilon)$
rounds~\cite{DBLP:conf/isaac/GoodrichSZ11}.  The input is a sequence
of tuples $\{t_1, \ldots, t_N\}$, an associative binary operator
$\oplus$, and an identity element, $\bot$.  The output is a sequence
of tuples $S$, s.t. $S_j$ is equal to $t_j$, with an extra entry
containing $\bot \oplus_{i=1}^{j-1} t_j$. Note that reductions are a
special case of prefix sums.

\item {\bf Predecessor.} The predecessor problem on a sequence of $N$
tuples can be solved in $O(1/\epsilon)$
rounds~\cite{DBLP:conf/isaac/GoodrichSZ11,andoniparallel}.  The input
is a sequence of $N$ tuples, where each tuple has an associated value
in $\{0, 1\}$. The problem is to compute for each tuple $x$, the first
tuple $x'$ that appears before $x$ in the sequence s.t. $x'$ has an
associated value of $1$.

\item {\bf Duplicate Removal.} Given a sequence of $N$ elements, we
can remove duplicates in the sequence in $O(1/\epsilon)$ rounds by
simply sorting the elements and removing any tuple that is identical
to the one before it, using predecessor.

\item {\bf Range Minimum Query.} Given a sequence of $n$ elements,
a range minimum query (RMQ) data structure enables efficiently
querying for the minimum value element between a range $[i, j]$.
Andoni et al.~\cite{andoniparallel} give a data structure that
builds an RMQ data structure using $O(1/\epsilon)$ rounds of \MPC{},
which can then be used to answer queries in $O(1)$ rounds.

\item {\bf Graph Contraction.} Given a graph $G = (V, E)$ and a
mapping $f : V \rightarrow S$ where $S \subseteq V$, contracting the
graph to $(S, \{(f(u), f(v))\ |\ (u, v) \in E\})$ can be done in
$O(1)$ rounds of \AMPC{}. We first store the mapping $f$ in the DDS.
Next, we map the set of edges to $(f(u), f(v))$ using two queries per
edge. Finally, we remove duplicates from the edge set.

\end{itemize}

\subsection{Algorithm Implementations}

We now describe how the algorithms described in this paper can be
implemented in the \AMPC{} model in the required number of rounds.

\myparagraph{2-Cycle}
Algorithm~\ref{alg:shrink} can be implemented in $O(1)$ rounds by
first storing the sampled vertices in the DDS. As we traverse the
cycle for a given vertex, we also issue queries to check whether the
neighbor is a sampled vertex, which increases the number of queries by
a constant factor (an alternate implementation is to sample vertices
using a hash function, which eliminates the need for these queries.).
Since the \twocycle{} algorithm simply calls
Algorithm~\ref{alg:shrink} $O(1/\epsilon)$ times, \twocycle{} can be
implemented in $O(1/\epsilon)$ rounds of \AMPC{}.

\myparagraph{Maximal Independent Set}
To simulate $\pi$ it suffices to sample a random priority between $[0,
1]$ for each vertex. We preprocess the graph by sorting each neighbor
list with respect to the samples, and store the preprocessed graph in
the DDS. The keys stored are pairs of a node and index, $(v, i)$,
which stores the value of the $i$th lightest neighbor incident on $v$.

We now show that each step in an iteration of the loop in \mis{} can
be implemented in $O(1)$ rounds of \AMPC{}.  Each iteration of the
loop just applies \truncatedquery{} to each vertex assigned to the
machine whose status is still unknown until \truncatedquery{} fails to
settle some vertex. It is easy to see that if the \truncatedquery{}
algorithm performs $q$ queries, then this results in $O(q)$ queries
that are sent to the DDS.

\myparagraph{Connectivity}
Consider the steps in the main loop of the algorithm.
\increasedegree{} can be implemented in $O(1)$ rounds of \AMPC{}
since the query performed for each vertex can be sequentially run
within $1$ round.
Sampling the vertices as leaders can be done in $1$ round.
Next, contracting $G$ to $G'$ can be done in $O(1)$ rounds as follows.
First we use a reduce to collect the lowest-id leader incident on each
vertex. In the next step, we collect the lowest-id vertex incident on
the vertex, again by reducing over the edges incident on each vertex.
If the degree of a vertex is at least $d$, but it has no leader
incident on it (and is not itself a leader), then we can terminate the
algorithm (note that this event happens with probability $1/n^{c}$ for
an arbitrarily large constant $c$).
Finally, contracting the graph to the leaders can be done in $O(1)$
rounds.
Updating $M$ can be done in $O(1)$ rounds by storing $M'$ in the DDS
and querying for the value $M(v)$ in $M'$ for each vertex $v \in V$
mapped to $M(v)$.

Therefore, each iteration of the main loop can be implemented in
$O(1)$ rounds of \AMPC{}, and the algorithm can be implemented in
$O(\log\log_{T/n} n)$ rounds of \AMPC{} w.h.p.

\myparagraph{Minimum Spanning Forest}
Since the algorithm is very similar to our \connectivity{} algorithm,
we focus on the main differences. First, note that efficiently
implementing Prim's algorithm requires iterating over the neighbors of
a vertex, sorted by weight. We can implement this by first sorting the
neighbors of each vertex by weight, and storing this preprocessed
graph in the DDS where the keys are pairs of a node and index, $(v,
i)$, which stores the $i$th lightest edge incident on $v$.

Now, we show that each iteration of the loop can be implemented in
$O(1)$ rounds.  \msfincreasedegree{} can then be implemented in $O(1)$
rounds since each vertex makes at most $d^2$ queries to the
preprocessed graph in the DDS before halting. We can remove duplicates
in order to compute the set of tree edges found in this round in
$O(1)$ round. Next, applying $M$ to recover the original edges can be
done in $O(1)$ rounds by storing $M$ in the DDS and querying in
parallel for each edge. Sampling and contracting can be done in $O(1)$
rounds by the same argument as the connectivity algorithm.

Since each iteration of the main loop can be implemented in $O(1)$
rounds of \AMPC{}, our minimum spanning forest algorithm can be
implemented in $O(\log\log_{T/n} n)$ rounds of \AMPC{} w.h.p.

\myparagraph{List Ranking}
The list ranking algorithm can be implemented similarly to the
\twocycle{} algorithm. As before, we store the sampled vertices in the
DDS. We also store all contracted graphs generated by the algorithm in
the DDS, which does not violate the total space since the algorithm
performs $O(1/\epsilon)$ rounds. Observe that the traversal in both
the first (contraction) and second (uncontraction) loops can be done
in $1$ round of \AMPC{} by issuing queries to the current graph stored
in the DDS. Furthermore, the contraction step in the first loop can be
implemented in $O(1)$ rounds using the graph contraction primitive.
Therefore, the algorithm runs in $O(1)$ rounds of \AMPC{} w.h.p. Note
that we

\myparagraph{Tree Operations}
\emph{Computing an Euler tour}
Computing the Euler tour of a tree given the tree edges can be done in
$O(1)$ rounds by first aggregating all edges incident to the vertex.
Next, the edges are stored in the DDS, along with their position
in the adjacency lists incident on both endpoints. An edge $e = (u,
u_i, v, v_i)$ where $u_i$ is its position in $u$'s list and $v_i$ is
its position in $v$'s list can then add pointers to its left and right
neighbors in the Euler tour using $2$ queries.

\emph{Rooting a Tree} can be done in $O(1/\epsilon)$ rounds by
applying the reduction described in Section~\ref{sec:treeoperations}.
Computing an Euler tour costs $O(1)$ rounds.  Computing list ranking
with respect to root costs $O(1/\epsilon)$ rounds w.h.p. as describe
above. Finally, identifying the forward and reverse edges can be done
by storing the edges and their ranks in the DDS and issuing a single
query per directed edge to its twin. At this point, we can label the
parent and child for each tree edge, and have therefore shown how to
root a tree in $O(1/\epsilon)$ rounds w.h.p.

\emph{Subtree Sizes and Preorder Numbering}
We first compute an Euler sequence and label edges as forward and
reverse edges, as described above. The first round maps over the edges
and assigns the weights. Next, we compute a prefix-sum which can be
done in $O(1)$ rounds. For subtree sizes, we store the prefix sums in
the DDS and issue two queries for each vertex to fetch the values at
the first and last occurrence of its incident edges. For preorder
numbering, we just return the value of the first occurrence of an edge
incident to the vertex. Both operations therefore run in
$O(1/\epsilon)$ rounds of \AMPC{}.

\myparagraph{2-Edge Connectivity}
Computing a spanning forest can be implemented in $O(\log\log_{T/n}
n)$ rounds w.h.p. based on the description above for computing a
minimum spanning forest. Furthermore, we can compute the connected
components in the same bounds to retrieve a mapping from vertices to
their component ids (the spanning forest algorithm can also be easily
modified to output this). Using this mapping, we can implement the
\textsc{RootForest} operation in terms of the tree rooting operation
above by first picking an arbitrary vertex per component and rooting
the tree at this vertex. Rooting can therefore be done in
$O(1/\epsilon)$ rounds w.h.p.

Now, computing the subtree functions on the rooted trees can each be
done in $O(1/\epsilon)$ rounds w.h.p.  based on the descriptions
above. Computing the critical edges can be done in $O(1)$ rounds by
first storing the values computed by the tree operations in the DDS
and making $O(1)$ queries per edge. Finally, computing connectivity on
the graph with the critical edges removed can be done in
$O(\log\log_{T/n} n)$ rounds w.h.p. based on the description for
connectivity above.

Queries to the BC-labeling, can be done by storing the BC-labeling in
the DDS. The 2-edge connected component queries requires $O(m)$ total
queries to determine the bridges. The last step is another call to
connectivity which runs in the required round complexity. It is simple
to verify that each of the steps above runs in $O(T)$ space.

\myparagraph{Forest Connectivity}
The forest connectivity algorithm works by first computing a set of
Euler tours over the forest. By the description above, computing the
tours can be done in $O(1)$ rounds of \AMPC{}. Next, the cycle
connectivity algorithm makes $O(1/\epsilon)$ calls to \shrink{}. By
the argument above for the \twocycle{} problem, each of these calls
runs in $O(1)$ rounds of \AMPC{}. Finally, we run the query-based
algorithm, which runs in $1$ round where each of the $O(n^{1 -
  \epsilon}\log n)$ machines make $O(n^{\epsilon})$ queries in total
w.h.p. Therefore, the algorithm can be implemented to run in
$O(1/\epsilon)$ rounds of \AMPC{}.



==> proofs.tex <==
\section{Proof of Lemma~\ref{lem:contention}}
\contention*

\begin{proof}
First we fix a certain bin $b$ and show that the total weight of the balls in that bin is $O(S)$ with high probability. Then we use a union bound to show it for all bins simultaneously.
For each ball $i\in \{1,\dots,T\}$ let $X_i$ be a random variable that is $0$ if ball $i$ is not in bin $b$ and be equal to the weight of ball $i$ otherwise. Let $X = \sum_{i=1}^T X_i$ and note that $E[X]= \frac T P = S$. By the standard Bernstein's inequality we have 
\begin{align*}
    P\Big(\big|X-E[X]\big|\leq E[X]\Big) &\leq \exp\Big(-\frac{E[X]^2/2}{\mathsf{Var}(X)+P E[X]/3}\Big) \\&\leq  \exp\Big(-\frac{S^2}{2 \mathsf{Var}(X) +P S}\Big),
\end{align*}
where $\mathsf{Var}(X)$ is the variance of the random variable $X$. Next, we bound $V$. Let $p_i$ be the weight of ball $i$. We have
\begin{align*}
    \mathsf{Var}(X) &= \sum_{i=1}^T \mathsf{Var}(X_i) = \sum_{i=1}^T \big(\frac{1}{P}(1-\frac{1}{P})p_i^2\big)\\
    &\geq \frac{1}{P} \sum_{i=1}^T p_i^2 \leq \frac{1}{P} \max(p_i) \sum_{i=1}^T p_i\\
    &= \frac{1}{P} \cdot P \cdot T = T.
\end{align*}
Therefore we have 
\begin{align*}
    P\Big(\big|X-E[X]\big|\leq E[X]\Big) \leq  \exp\Big(-\frac{S^2}{2 T +P S}\Big) = \exp\big(-P^{\Omega(1)}\big),
\end{align*}
which concludes the proof.
\end{proof}



==> smalltotalspace.tex <==
\section{Handling Instances with $T \leq 10 n \log^2 n$}\label{sec:smalltotalspace}

In this section, show how to shrink the number of vertices of the input graph by a $\log^2 n$ factor without changing its connectivity structure. This releases enough total space for our algorithms to assume that $m = \Omega(n \log^2 n)$.
We note that the contents of this section have been copied from another manuscript by the authors and are provided for completeness of our algorithm.

\smalltotalspace*
\begin{proof}
	In order to prove this lemma, we show that the following procedure reduces the number of vertices of the graph by a constant factor, with high probability. This procedure only merges some neighboring vertices and hence maintains the connected components. In this procedure, without loss of generality, we assume that there is no isolated vertices. One can simply label and remove all isolated vertices at the beginning.
	It is easy to implement this procedure in $\frac 1 {\delta}$ rounds using $O(n^{\delta})$ space per machine and a total space of $O(m)$. Repeating this procedure $O(\log\log n)$ times (and doing a union bound over all runs) proves the lemma. Note that in the case where $T \leq n \polylog n$ we have $ \log \log_{T/n} n = O(\log \frac {\log n}{\log\log n}) = O(\log \log n)$.

\begin{tboxalg}{An algorithm to shrink the number of vertices by a constant factor in $O(1)$ rounds w.h.p.}\label{alg:shrinkvertices}
	\begin{enumerate}[ref={\arabic*}, topsep=0pt,itemsep=0ex,partopsep=0ex,parsep=1ex, leftmargin=*]
		\item For each vertex $v$, draw a directed edge from $v$ to its neighbor with the minimum id. \label{line1}
		\item If for two vertices $u$ and $v$, we drew two directed edges $(u,v)$ and $(v,u)$, we remove one arbitrary. \label{line2}
		\item If a vertex has more than one incoming edge, we remove its outgoing edge.\label{line3}
		\item If a vertex $v$ has more than one incoming edge, we merge it with all its neighbors (via directed edges) and remove the incoming directed edges of the neighbors of $v$.\label{line4}
		\item We remove each edge with probability $2/3$.\label{line5}
		\item We merge each directed isolated edge.\label{line6}
	\end{enumerate}
\end{tboxalg}

Next we show that this procedure reduces the number of vertices by a constant factor. For readability, we do not optimize this constant. 
Note that in Line \ref{line1} we are adding $n$ edges. It is easy to see that there is no cycle of length larger than $2$ in the directed graph constructed in Line \ref{line1}. Line \ref{line2} removes at most half of the edges. Moreover, it removes all cycles of length $2$. Thus by the end of Line \ref{line2} we a rooted forest with at least $n/2$ edges. 

After Line \ref{line3} every vertex with indegree more than $1$ has no outgoing edges. Recall that each vertex has at most one outgoing edge. Thus, after Line \ref{line3} we have a collection of rooted trees where only the root may have degree more than $2$. We call such trees \emph{long tail stars}. Note that if we remove the outgoing edge of a vertex $v$ there are two incoming edges pointing to $v$ (which uniquely correspond to $v$). Although the process of Line \ref{line3} may cascade and remove the incoming edges of $v$, the following simple double counting argument bounds the number of removed edges. Note that this argument is just to bound the number of the edges and we do not require to run it, in order to execute our algorithm.

We put a token on each directed edge of the forest (before running Line \ref{line3}). Next we are going to move the tokens such that (a) we never have more than two tokens on each edge, and (b) at the end we move all tokens to the edges that survive after Line \ref{line3}. This says that at least half of the edges (i.e., at least $n/4$ edges) survive Line \ref{line3}.

We traverse over each rooted tree from the root to the leaves. At each step, if the outgoing edge of a vertex $v$ is removed, by induction hypothesis there are at most two tokens on the edge. Also, $v$ has at least two incoming edges. We move each of the tokens on the outgoing edge of $v$ to one of its incoming edges. Note that this is the only time we move a token to the incoming edges of $v$ and hence we do not have more than two tokens on each edge as desired.

If we merge a vertex $v$ with $r$ incoming edges in Line \ref{line4}, we remove at most $2r$ directed edges ($r$ incoming edges of $v$ and at most one incoming edge per each neighbor of $v$. On the other hand, we decrease the number of vertices by $r$. Thus, if this stage removes more than $n/8$ edges the number of vertices drops to at most $n-\frac n {16} = \frac{15}{16}n$, as desired. To complete the proof, we assume that at most $n/8$ edges are removed in Line \ref{line4} and show that in this case Lines \ref{line5} and \ref{line6} decrease the number of vertices by a constant factor.

Note that Line \ref{line4} removes the root of all long tailed stars. Thus after Line \ref{line4} we have a collection of directed edges. The probability that an edge passed to Line \ref{line5} become an isolated edge after sampling is at least $\frac 2 3 \cdot \frac 1 3 \cdot \frac 2 3 = \frac 4 {27}$. If we mark every third edge (starting from an end of each path), the chance that each marked edge becomes an isolated edge after sampling is independent of other marked edges. There are $\frac 1 3 \cdot \frac n 8 = \frac n {24}$ marked edges. Let $X$ be a random variable that indicates the number of marked edges that are isolated after sampling. Note that $\E[X]\geq \frac{4}{27}\frac{n}{24}=\frac n {162}$. By applying a simple Chernoff bound we have
\begin{align*}
\Pr\Big[X \leq  0.5 \frac n {162}\Big] \leq \exp \Big(-\frac{0.5^2 \frac n {162}}{2}\Big) 
=  \exp \Big(-\frac{n}{1296}\Big).
\end{align*}
Therefore, with high probability we merge at least $\frac{n}{324}$ edges in Line \ref{line6} as desired. 
\end{proof}




==> tree-operations.tex <==
\section{Tree Operations}\label{sec:treeoperations}

\myparagraph{Subtree Sizes}
Given a rooted tree, $T$, we show how to compute the subtree sizes for
each vertex in the tree. We first compute the Euler sequence of $T$,
starting at the root. Next we assign a weight of $1$ to each forward
edge and a weight of $0$ to each reverse edge (see the discussion on
rooting trees above). Computing a prefix-sum over the Euler sequence
with respect to the weights computes, for each edge, the number of
forward edges preceding it. The subtree size at a given node, $v$, can
be obtained by taking the difference of the values for the last
reverse edge entering $v$ and the first forward edge exiting $v$.
Therefore, we have the following lemma:
\begin{lemma}\label{lem:subtreesizes}
Computing the subtree sizes of a rooted tree can be performed in
$O(1/\epsilon)$ rounds of $\AMPC{}$ w.h.p. using $O(N)$ total space
w.h.p.
%Furthermore, the algorithm
%uses $O(n^{\epsilon})$ queries per machine w.h.p.
\end{lemma}

\myparagraph{Preorder Numbering}
Computing a preorder numbering of a rooted tree can also be done using
the Euler sequence and prefix-sums. The idea is similar to the subtree
size algorithm. We store a weight of $1$ for each forward edge and a
weight of $0$ for each reverse edge, and compute the prefix-sum over
the weighted Euler sequence with respect to the weights. The preorder
number of a vertex is simply the number of forward edges preceding it.
Therefore, we have the following lemma:
\begin{lemma}\label{lem:preordernumbering}
Computing the preorder numbering of a rooted tree can be performed in
$O(1/\epsilon)$ rounds of $\AMPC{}$ w.h.p. using $O(N)$ total space
w.h.p.
% Furthermore, the algorithm
% uses $O(n^{\epsilon})$ queries per machine w.h.p.
\end{lemma}

\myparagraph{Subtree Minimum and Maximum}
Note that the Euler tour based technique described above to compute
subtree sizes is not sufficient to compute the minimum and maximum
over subtrees quickly (the technique depends on the function having an
inverse, which precludes using it for $\min, \max$). The classic
solution to this problem is the range minimum query (RMQ) data
structure. The data structure is built over an input array of $n$
elements. Queries take two indices, $i, j$ and return the minimum
value element in this range. Observe that after computing the Euler
sequence, computing the minimum and maximum of a vertex $v$'s subtree
can be reduced to a RMQ on the interval in the Euler tour representing
$v$'s subtree. Using the fact that RMQ can be implemented efficiently
in the \MPC{} setting (see Appendix~\ref{apx:implementation-details}) gives us
the following lemma:
\begin{lemma}\label{lem:subtreeminmax}
A data structure to compute the minimum and maximum of a subtree can
be computed in $O(1/\epsilon)$ rounds of \AMPC{}. Each query to the data structure can be answered in $O(1)$ rounds.
Preprocessing and storing the data structure uses $O(N)$ total space w.h.p.
%Furthermore, the algorithm uses
%$O(n^{\epsilon})$ queries per machine.
\end{lemma}







%% \section{Spanning Forest and Tree Operations}
%%
%% In this section we show how to extend our undirected connectivity
%% algorithm to compute a spanning forest of the graph. We also give
%% primitives for rooting trees, list ranking, computing subtree sizes
%% and finding a preorder numbering of a tree.
%%
%% \myparagraph{Spanning Forest}
%% At a high level, our spanning forest algorithm is similar to the
%% undirected connectivity algorithm in Section~\ref{sec:connectivity}.
%% However, obtaining a spanning forest algorithm requires making a few
%% small but important modifications. The first issue that arises is how
%% to select leaders to contract to in a way that lets us incrementally
%% build a spanning forest of the graph. Our approach is to modify each
%% iteration to find a set of tree edges and contract the graph based on
%% these tree edges. This step ensures that two vertices are contracted
%% to the same vertex if and only if there is a path along tree edges
%% that have already been added to the spanning forest.
%%
%% Another issue encountered when modifying
%% Algorithm~\ref{alg:connectivity} is the fact that the edges added to
%% the graph by the \increasedegree{} procedure are not edges actually
%% present in the original graph. We refer to these edges which are
%% added to increase a vertex's degree as \emph{virtual edges}, and refer
%% to edges in the graph corresponding to some original edge in the graph
%% as \emph{real edges}. Our goal in each iteration of the algorithm is
%% for each vertex $v$, to (1) select a vertex to contract to and (2) to
%% select a real edge so that there is a path along real edges chosen in
%% this iteration that connect $v$ to the leader it contracts to.
%%
%% Our approach is to modify the \increasedegree{} procedure to output a
%% set of weighted edges where the weight of each edge is the distance in
%% between the root of the BFS and the new neighbor. After running the
%% modified procedure, each real edges in the graph has a weight of $1$,
%% and every virtual edge has a distance greater than $1$.
%% Then, in the contraction step, each vertex first emits its distance to
%% the closest leader, and the id of the leader. If a vertex is directly
%% connected to a leader by a real edge, it selects this real edge,
%% contracts to the leader and quits. Otherwise, the vertex scans its
%% neighbors and selects the edge to its neighbor that is closest to a
%% leader, and selects the neighbors' leader to contract to.  Note that
%% we delete all virtual edges before contracting the graph, to ensure
%% that only real edges persist in the contracted graph.
%%
%% Algorithm~\ref{alg:increase-degree-sf} gives our modified
%% \increasedegree{} algorithm, \increasedegreesf{} and
%% Algorithm~\ref{alg:spanning-forest} gives our spanning forest
%% algorithm.
%%
%% \begin{tboxalg}{$\increasedegreesf(G=(V, E), d)$}\label{alg:increase-degree-sf}
%% 	\begin{enumerate}[ref={\arabic*}, topsep=0pt,itemsep=0ex,partopsep=0ex,parsep=1ex, leftmargin=*]
%%     \item Assign the currently active vertices to the machines
%%       uniformly at random.
%%
%%     \item Each machine runs a BFS for each vertex, $v$, assigned to
%%       it, where neighboring vertices are visited consistently (e.g.,
%%       sorted by their ids). Add a weighted edge between $v$ and a
%%       newly discovered vertex $u$ with weight equal to $d_{G}(v, u)$.
%%       Terminate the BFS once $v$'s degree is $\geq d$, or all vertices
%%       in the component containing $v$ are discovered.
%%
%%     \item Output $G' = (V, E')$ where $E'$ contains both $E$ and the
%%       newly discovered edges.
%% 	\end{enumerate}
%% \end{tboxalg}
%%
%% \begin{tboxalg}{\spanningforest{}(G=(V, E))}\label{alg:spanning-forest}
%% 	\begin{enumerate}[ref={\arabic*}, topsep=0pt,itemsep=0ex,partopsep=0ex,parsep=1ex, leftmargin=*]
%%
%%     \item Let $n = |V|, G_{C} = G, E_{T} = \emptyset$, and $M_{E}$ be
%%       a mapping from the edges of $G_{C}$ to $E$.
%%
%%     \item If $m = o(n\log^2 n)$, let $G_C$ be result of applying
%%     Corollary~\ref{cor:handlesparse} to reduce the number of vertices
%%     to $O(n/\log^2 n)$. Add the tree edges found in this step to
%%     $E_{T}$. \label{sf:handlesparse}
%%
%%     \item Let $d' = \max(T/n, \log^2 n)$, and $d = \sqrt{d'}$.
%%
%%     \item While $G_{C}$ is non-empty, perform the following
%%       steps:\label{sf:loopstart}
%%
%%     \begin{enumerate}
%%       \item Randomly assign the vertices in $G_C$ to machine and call
%%         $\increasedegreesf{}(G_C, d)$ for each vertex. Add the weighted
%%         edges found to $G_C$.\label{sf:increasedegree}
%%
%%       \item Sample each vertex with probability $O(\log n / d)$ to be
%%         a leader.
%%         \label{step:sampleleaders}
%%
%%       \item For each vertex, $v$ let $(d(v), l(v))$ be the distance
%%         and id of the closest leader to $v$ (choosing the lowest id
%%         leader to break ties). If $d(v) = 1$, add $M_{E}[(v, l(v))]$
%%         to $E_{T}$. Otherwise, add the edge $M_{E}[(v, n(v))]$ to
%%         $E_{T}$ where $n(v)$ is a neighbor of $v$ satsifying
%%         $d_{G}(v, l(v)) = 1 + d_{G}(n(v), l(v))$.
%%         \label{step:selectleaderandedge}
%%
%%       \item Let $G'$ be the graph formed by first dropping all virtual
%%         edges from $G_{C}$, and then contracting each vertex, $v$ to
%%         $l(v)$. Update $M_{E}$ to map $e \in E(G')$ to $M_{E}(e')$
%%         where $e'$ is some edge in $G_{C}$ corresponding to $e$ in the
%%         contracted graph.
%%
%%       \item Update $d = \max(d^{1.5}, n^{\epsilon/2})$ and $d' =
%%         \max(d'^{1.5}, n^{\epsilon})$ and $G_{C} = G'$.
%%
%%     \end{enumerate}
%%     \item Output $E_{T}$
%% 	\end{enumerate}
%% \end{tboxalg}
%%
%% \begin{lemma}\label{lem:consistentvirtual}
%% Consider an iteration of the loop in Step~\ref{sf:loopstart}. Let
%% $E_{r}$ be the set of real edges in $G_{C}$ found in this iteration.
%% For each $v \in G_{C}$ that is not selected as a leader, there is a
%% path consisting of 1 or more edges from $E_{r}$ to its chosen leader.
%% \end{lemma}
%% \begin{proof}
%% The proof is by induction on the distance, $d$, to its closest leader.
%% Specifically, we show that if a non-leader vertex $v$ selects $l(v)$
%% as its leader and adds the real edge $(v, u)$ where $u \in N(v)$, then
%% $l(u) = l(v)$ and also there is a path $P = \{(v, u), \ldots, e_k\}$
%% of real edges connecting $v$ to $l(v)$. When $d=1$, $v$ adds the real
%% edge $(u, l(v))$ proving the base case since $l(l(v)) = l(v)$.
%%
%% Now, suppose $d > 1$ and inductively assume that the statement holds
%% for $d' < d$. Let $(v, u)$ be the real edge chosen by $v$. Notice that
%% since $v$'s BFS performed during \increasedegreesf{} goes through $u$, it
%% will query a subset of the vertices explored by $u$'s BFS.
%% Furthermore, since the BFSs are performed consistently, and any ties
%% between leaders at the same level in the BFS tree are broken
%% consistently, a simple proof by contradiction shows that if $v$'s
%% shortest path to $l(v)$ goes through $u$, then $u$ must also be
%% connected to $l(v)$ in $G_{C}$.
%%
%% Therefore, Step~\ref{step:selectleaderandedge} will find such a vertex
%% $u$, and we have that $l(v) = l(u)$. By our induction hypothesis, we
%% have that $u$ is connected to $l(v)$ by some path of real edges, $p_1,
%% \ldots, p_k$. Adding $(v, u)$ to this path produces a path of real
%% edges connecting $v$ to $l(v)$, finishing the proof.
%% \end{proof}
%%
%% \begin{lemma}\label{lem:sfcorrect}
%%   Algorithm~\ref{alg:spanning-forest} outputs a valid spanning forest
%%   of $G$.
%% \end{lemma}
%% \begin{proof}
%% The steps before the start of the loop on Step~\ref{sf:loopstart} are
%% correct due to Lemma~\ref{lem:smalltotalspace}. The proof is by
%% induction on the number of iterations. We will show that after each
%% iteration, $E_{T} \cup M_{E}(SF(G_{C}))$ is a valid spanning forest of
%% $G$.
%%
%%
%% \end{proof}
%%
%% \begin{lemma}\label{lem:sfcorrect}
%%   Algorithm~\ref{alg:spanning-forest} runs in $O(\log\log_{T/n} n)$
%%   rounds w.h.p. where in each round, each machine performs
%%   $O(n^{\epsilon})$ queries w.h.p.
%% \end{lemma}
%% \begin{proof}
%%   The proof of the round-complexity and query-complexity is almost
%%   identical to the proof of Theorem~\ref{thm:connectivity-rounds}.
%% \end{proof}

